A posteriori error analysis of the virtual element method for second-order quasilinear elliptic PDEs

In this paper we develop a $C^0$-conforming virtual element method (VEM) for a class of second-order quasilinear elliptic PDEs in two dimensions. We present a posteriori error analysis for this problem and derive a residual based error estimator. The estimator is fully computable and we prove upper and lower bounds of the error estimator which are explicit in the local mesh size. We use the estimator to drive an adaptive mesh refinement algorithm. A handful of numerical test problems are carried out to study the performance of the proposed error indicator.

==> Setup/packagesCMAM.tex <==
% \usepackage[english]{babel}
% \usepackage[a4paper]{geometry}
% \usepackage[utf8]{inputenc}
% \usepackage{hyperref}
% \usepackage{amsfonts}
% % \usepackage{caption}
% \usepackage{amsthm}
% \usepackage{amsmath}
\usepackage{graphicx}
% \usepackage{amssymb}
% \usepackage{enumerate}
\usepackage{xfrac}
\usepackage{array}
\usepackage{siunitx}
\usepackage{mathtools}
\usepackage{mathrsfs}
\usepackage{enumitem}
\setlist[enumerate]{topsep=0pt}
\setlist[itemize]{topsep=0pt}
\usepackage{float}
\usepackage[nodayofweek]{datetime} 
\usepackage[framemethod=tikz]{mdframed}
\usepackage{tikz}
\graphicspath{ {images/} }
% \usepackage{listings}
\usepackage{color}
% \usepackage[draft]{todonotes} 
\usepackage{comment}
\usepackage{stmaryrd}
\usepackage{bm}
\usepackage{pgfplots}
\pgfplotsset{compat=1.18}

\usepackage{nicefrac}

\usepackage{placeins}
\usepackage{subfig}

==> new_results/problem1.tex <==
% quads figure
\begin{figure}
  % row 1
  \begin{center}
    \begin{subfigure}{0.49\textwidth}
      \begin{tikzpicture}
        \begin{loglogaxis}[
            width=0.9\linewidth,
            label style={font=\small},
            tick label style={font=\small},
            grid=major, % Display a grid
            grid style={dashed,gray!20}, % Set the style
            xlabel={Number of degrees of freedom}, % Set the labels
            ylabel={$\| \nabla u - \gradProj u_h \|_{0,\Omega}$ },
            legend style={anchor=north east, nodes={scale=0.75, transform shape}},
            % mark repeat=100,
            mark phase=0,
            mark size=1.5,
            cycle list name=mylist,
            % log ticks with fixed point,
            % xtick={100, 1000, 10000},
            % xticklabels={$10^2$, $10^3$, $10^4$
            % },
          ]
          \addplot+[] table[x=dofs,y=H1 error,col sep=comma] {new_results/problem1/problem1_quads_p1.csv};
          \addplot+[] table[x=dofs,y=H1 error,col sep=comma] {new_results/problem1/problem1_quads_p2.csv};
          \addplot+[] table[x=dofs,y=H1 error,col sep=comma] {new_results/problem1/problem1_quads_p3.csv};
        %   \addplot+[domain=100:5000, samples=4, gray, dashed, no markers] {x^(-0.5)}; 
        %   \addplot+[domain=100:5000, samples=4, gray, dashed, no markers] {x^(-1)}; 
        %   \addplot+[domain=100:5000, samples=4, gray, dashed, no markers] {x^(-1.5)}; 
          \legend{$\polOrder=1$,$\polOrder=2$,$\polOrder=3$}
        \end{loglogaxis}
      \end{tikzpicture}
      \caption{}
    \end{subfigure}
    % \quad
    \begin{subfigure}{0.49\textwidth}
      \begin{tikzpicture}
        \begin{loglogaxis}[
            width=0.9\linewidth, % Scale the plot to \linewidth
            label style={font=\small},
            tick label style={font=\small},
            grid=major, % Display a grid
            grid style={dashed,gray!20}, % Set the style
            xlabel={Number of degrees of freedom}, % Set the labels
            ylabel={Estimator of $\| \nabla u - \gradProj u_h \|_{0,\Omega}$ },
            legend style={anchor=north east, nodes={scale=0.75, transform shape}},
            % mark repeat=100,
            mark phase=0,
            mark size=1.5,
            cycle list name=mylist,
            % log ticks with fixed point,
            % xtick={100, 1000, 10000},
            % xticklabels={$10^2$, $10^3$, $10^4$
            % },
          ]
          \addplot+[] table[x=dofs,y=Estimated error,col sep=comma] {new_results/problem1/problem1_quads_p1.csv};
          \addplot+[] table[x=dofs,y=Estimated error,col sep=comma] {new_results/problem1/problem1_quads_p2.csv};
          \addplot+[] table[x=dofs,y=Estimated error,col sep=comma] {new_results/problem1/problem1_quads_p3.csv};
        %   \addplot+[domain=100:5000, samples=4, gray, dashed, no markers] {x^(-0.5)}; 
        %   \addplot+[domain=100:5000, samples=4, gray, dashed, no markers] {x^(-1)}; 
        %   \addplot+[domain=100:5000, samples=4, gray, dashed, no markers] {x^(-1.5)}; 
          \legend{$\polOrder=1$,$\polOrder=2$,$\polOrder=3$}
        \end{loglogaxis}
      \end{tikzpicture}
      \caption{}
    \end{subfigure}
  \end{center}

  % row 2  
  \begin{center}
    \begin{subfigure}{0.49\textwidth}
      \begin{tikzpicture}
        \begin{semilogxaxis}[
            width=0.9\linewidth, % Scale the plot to \linewidth
            label style={font=\small},
            tick label style={font=\small},
            grid=major, % Display a grid
            grid style={dashed,gray!20}, % Set the style
            xlabel={Number of degrees of freedom}, % Set the labels
            % ymin=0,
            % ymax=25,
            ylabel=Effectivity,
            legend style={at={(1,1)}, anchor=north west, nodes={scale=0.75, transform shape}},
            % mark repeat=100,
            mark phase=0,
            mark size=1.5,
            cycle list name=mylist,
            % log ticks with fixed point,
            % xtick={100, 1000, 10000},
            % xticklabels={$10^2$, $10^3$, $10^4$
            % },
          ]
          \addplot+[] table[x=dofs,y=Effectivity,col sep=comma] {new_results/problem1/problem1_quads_p1.csv};
          \addplot+[] table[x=dofs,y=Effectivity,col sep=comma] {new_results/problem1/problem1_quads_p2.csv};
          \addplot+[] table[x=dofs,y=Effectivity,col sep=comma] {new_results/problem1/problem1_quads_p3.csv};
          \legend{$\polOrder=1$,$\polOrder=2$,$\polOrder=3$}
        \end{semilogxaxis}
      \end{tikzpicture}
      \caption{}
    \end{subfigure}
  \end{center}

  % row 3
  \begin{center}
    \begin{subfigure}{0.3\textwidth}
      \includegraphics[trim={3.5cm 0.5cm 3cm 0.5cm},clip, width=0.9\linewidth]{new_results/problem1/problem1_quads_p1_level0.eps}
      \caption{Initial quadrilateral grid.}
      \label{fig: prob1 quads step 0}
    \end{subfigure}
    \quad
    \begin{subfigure}{0.3\textwidth}
      \includegraphics[trim={3.5cm 0.5cm 3cm 0.5cm},clip, width=0.9\linewidth]{new_results/problem1/problem1_quads_p1_level15.eps}
      \caption{After 15 refinements.}
    \end{subfigure}
    \quad
    \begin{subfigure}{0.3\textwidth}
      \includegraphics[trim={3.5cm 0.5cm 3cm 0.5cm},clip, width=0.9\linewidth]{new_results/problem1/problem1_quads_p1_level26.eps}
      \caption{After 26 refinements.}
      \label{fig: prob1 quads step 26}
    \end{subfigure}
  \end{center}

  \caption{Results from solving problem 1 on the quadrilateral grid with adaptive refinement. Figures~\ref{fig: prob1 quads step 0}-\ref{fig: prob1 quads step 26} show three different stages of the mesh sequence for $\polOrder=1$. }
  \label{fig: prob1 quads}
\end{figure}

% voronoi figure
\begin{figure}
  % row 1
  \begin{center}
    \begin{subfigure}{0.49\textwidth}
      \begin{tikzpicture}
        \begin{loglogaxis}[
            width=0.9\linewidth,
            label style={font=\small},
            tick label style={font=\small},
            grid=major, % Display a grid
            grid style={dashed,gray!20}, % Set the style
            xlabel={Number of degrees of freedom}, % Set the labels
            ylabel={$\| \nabla u - \gradProj u_h \|_{0,\Omega}$ },
            legend style={anchor=north east, nodes={scale=0.75, transform shape}},
            % mark repeat=100,
            mark phase=0,
            mark size=1.5,
            cycle list name=mylist,
            % log ticks with fixed point,
            % xtick={100, 1000, 10000},
            % xticklabels={$10^2$, $10^3$, $10^4$
            % },
          ]
          \addplot+[] table[x=dofs,y=H1 error,col sep=comma] {new_results/problem1/problem1_voronoi_p1.csv};
          \addplot+[] table[x=dofs,y=H1 error,col sep=comma] {new_results/problem1/problem1_voronoi_p2.csv};
          \addplot+[] table[x=dofs,y=H1 error,col sep=comma] {new_results/problem1/problem1_voronoi_p3.csv};
        %   \addplot+[domain=100:5000, samples=4, gray, dashed, no markers] {x^(-0.5)}; 
        %   \addplot+[domain=100:5000, samples=4, gray, dashed, no markers] {x^(-1)}; 
        %   \addplot+[domain=100:5000, samples=4, gray, dashed, no markers] {x^(-1.5)}; 
          \legend{$\polOrder=1$,$\polOrder=2$,$\polOrder=3$}
        \end{loglogaxis}
      \end{tikzpicture}
      \caption{}
    \end{subfigure}
    % \quad
    \begin{subfigure}{0.49\textwidth}
      \begin{tikzpicture}
        \begin{loglogaxis}[
            width=0.9\linewidth, % Scale the plot to \linewidth
            label style={font=\small},
            tick label style={font=\small},
            grid=major, % Display a grid
            grid style={dashed,gray!20}, % Set the style
            xlabel={Number of degrees of freedom}, % Set the labels
            ylabel={Estimator of $\| \nabla u - \gradProj u_h \|_{0,\Omega}$ },
            legend style={anchor=north east, nodes={scale=0.75, transform shape}},
            % mark repeat=100,
            mark phase=0,
            mark size=1.5,
            cycle list name=mylist,
            % log ticks with fixed point,
            % xtick={100, 1000, 10000},
            % xticklabels={$10^2$, $10^3$, $10^4$
            % },
          ]
          \addplot+[] table[x=dofs,y=Estimated error,col sep=comma] {new_results/problem1/problem1_voronoi_p1.csv};
          \addplot+[] table[x=dofs,y=Estimated error,col sep=comma] {new_results/problem1/problem1_voronoi_p2.csv};
          \addplot+[] table[x=dofs,y=Estimated error,col sep=comma] {new_results/problem1/problem1_voronoi_p3.csv};
        %   \addplot+[domain=100:5000, samples=4, gray, dashed, no markers] {x^(-0.5)}; 
        %   \addplot+[domain=100:5000, samples=4, gray, dashed, no markers] {x^(-1)}; 
        %   \addplot+[domain=100:5000, samples=4, gray, dashed, no markers] {x^(-1.5)}; 
          \legend{$\polOrder=1$,$\polOrder=2$,$\polOrder=3$}
        \end{loglogaxis}
      \end{tikzpicture}
      \caption{}
    \end{subfigure}
  \end{center}

  % row 2  
  \begin{center}
    \begin{subfigure}{0.49\textwidth}
      \begin{tikzpicture}
        \begin{semilogxaxis}[
            width=0.9\linewidth, % Scale the plot to \linewidth
            label style={font=\small},
            tick label style={font=\small},
            grid=major, % Display a grid
            grid style={dashed,gray!20}, % Set the style
            xlabel={Number of degrees of freedom}, % Set the labels
            % ymin=0,
            % ymax=25,
            ylabel=Effectivity,
            legend style={at={(1,1)}, anchor=north west, nodes={scale=0.75, transform shape}},
            % mark repeat=100,
            mark phase=0,
            mark size=1.5,
            cycle list name=mylist,
            % log ticks with fixed point,
            % xtick={100, 1000, 10000},
            % xticklabels={$10^2$, $10^3$, $10^4$
            % },
          ]
          \addplot+[] table[x=dofs,y=Effectivity,col sep=comma] {new_results/problem1/problem1_voronoi_p1.csv};
          \addplot+[] table[x=dofs,y=Effectivity,col sep=comma] {new_results/problem1/problem1_voronoi_p2.csv};
          \addplot+[] table[x=dofs,y=Effectivity,col sep=comma] {new_results/problem1/problem1_voronoi_p3.csv};
          \legend{$\polOrder=1$,$\polOrder=2$,$\polOrder=3$}
        \end{semilogxaxis}
      \end{tikzpicture}
      \caption{}
    \end{subfigure}
  \end{center}

  % row 3
  \begin{center}
    \begin{subfigure}{0.3\textwidth}
      \includegraphics[trim={3.5cm 0.5cm 3cm 0.5cm},clip, width=0.9\linewidth]{new_results/problem1/problem1_voronoi_p1_level0.eps}
      \caption{Initial Voronoi grid.}
      \label{fig: prob1 voronoi step 0}
    \end{subfigure}
    \quad
    \begin{subfigure}{0.3\textwidth}
      \includegraphics[trim={3.5cm 0.5cm 3cm 0.5cm},clip, width=0.9\linewidth]{new_results/problem1/problem1_voronoi_p1_level15.eps}
      \caption{After 15 refinements.}
    \end{subfigure}
    \quad
    \begin{subfigure}{0.3\textwidth}
      \includegraphics[trim={3.5cm 0.5cm 3cm 0.5cm},clip, width=0.9\linewidth]{new_results/problem1/problem1_voronoi_p1_level24.eps}
      \caption{After 24 refinements.}
      \label{fig: prob1 voronoi step 24}
    \end{subfigure}
  \end{center}

  \caption{Results from solving problem 1 on the Voronoi grid with adaptive refinement. Figures~\ref{fig: prob1 voronoi step 0}-\ref{fig: prob1 voronoi step 24} show three different stages of the mesh sequence for $\polOrder=1$. }
  \label{fig: prob1 voronoi}
\end{figure}

==> new_results/uniform.tex <==
\begin{figure}[p]\centering
    \begin{tikzpicture}
        \begin{loglogaxis}[
            width=0.5\textwidth, % Scale the plot to \linewidth
            grid=major, % Display a grid
            grid style={dashed,gray!20}, % Set the style
            xlabel={Number of dofs}, % Set the labels
            ylabel=,
            legend style={at={(0.025,0.025)}, anchor=south west, nodes={scale=0.75, transform shape}},
            % mark repeat=100,
            mark phase=0,
            mark size=1.5,
            cycle list name=exotic,
            % log ticks with fixed point,
            % xtick={100, 1000, 10000},
            % xticklabels={$10^2$, $10^3$, $10^4$
            % },
          ]
          \addplot+[]
          table[x=dofs,y=H1 error,col sep=comma] {new_results/uniform_quads_p1.csv};
          \addplot+[]
          table[x=dofs,y=H1 error,col sep=comma] {new_results/uniform_quads_p2.csv};
          \addplot+[]
          table[x=dofs,y=H1 error,col sep=comma] {new_results/uniform_quads_p3.csv};
          % \addplot+[]
          % table[x=dofs,y=Estimated error,col sep=comma] {results/uniform_testing_nonlinear_oldestimator_p2.csv};
          % \addplot+[domain=100:5000, samples=4, gray, dashed, no markers] {x^(-0.5)}; 
          % \addplot+[domain=100:5000, samples=4, gray, dashed, no markers] {x^(-1)}; 
          % \addplot+[domain=100:5000, samples=4, gray, dashed, no markers] {x^(-1.5)}; 
          \legend{$\polOrder=1$,$\polOrder=2$,$\polOrder=3$}
        \end{loglogaxis}
      \end{tikzpicture}
      \caption{Laplace problem 1: $H^1$-error with uniform refinement and original estimator method}
  \end{figure}
  
  \begin{figure}[p]\centering
    \begin{tikzpicture}
        \begin{loglogaxis}[
            width=0.5\textwidth, % Scale the plot to \linewidth
            grid=major, % Display a grid
            grid style={dashed,gray!20}, % Set the style
            xlabel={Number of dofs}, % Set the labels
            ylabel=,
            legend style={at={(0.025,0.025)}, anchor=south west, nodes={scale=0.75, transform shape}},
            % mark repeat=100,
            mark phase=0,
            mark size=1.5,
            cycle list name=exotic,
            % log ticks with fixed point,
            % xtick={100, 1000, 10000},
            % xticklabels={$10^2$, $10^3$, $10^4$
            % },
          ]
          \addplot+[]
          table[x=dofs,y=Estimated error,col sep=comma] {new_results/uniform_quads_p1.csv};
          \addplot+[]
          table[x=dofs,y=Estimated error,col sep=comma] {new_results/uniform_quads_p2.csv};
          \addplot+[]
          table[x=dofs,y=Estimated error,col sep=comma] {new_results/uniform_quads_p3.csv};
          % \addplot+[]
          % table[x=dofs,y=Estimated error,col sep=comma] {results/uniform_testing_nonlinear_oldestimator_p2.csv};
          % \addplot+[domain=100:5000, samples=4, gray, dashed, no markers] {x^(-0.5)}; 
          % \addplot+[domain=100:5000, samples=4, gray, dashed, no markers] {x^(-1)}; 
          % \addplot+[domain=100:5000, samples=4, gray, dashed, no markers] {x^(-1.5)}; 
          \legend{$\polOrder=1$,$\polOrder=2$,$\polOrder=3$}
        \end{loglogaxis}
      \end{tikzpicture}
      \caption{Laplace problem: estimated error with uniform refinement and original estimator method}
  \end{figure}
